Cognitive Endurance, Talent Selection, and the Labor Market Returns to Human Capital

Cognitive endurance -- the ability to sustain performance on a cognitively-demanding task over time -- is thought to be a crucial productivity determinant. However, a lack of data on this variable has limited researchers' ability to understand its role for success in college and the labor market. This paper uses college-admission-exam records from 15 million Brazilian high school students to measure cognitive endurance based on changes in performance throughout the exam. By exploiting exogenous variation in the order of exam questions, I show that students are 7.1 percentage points more likely to correctly answer a given question when it appears at the beginning of the day versus the end (relative to a sample mean of 34.3%). I develop a method to decompose test scores into fatigue-adjusted ability and cognitive endurance. I then merge these measures into a higher-education census and the earnings records of the universe of Brazilian formal-sector workers to quantify the association between endurance and long-run outcomes. I find that cognitive endurance has a statistically and economically significant wage return. Controlling for fatigue-adjusted ability and other student characteristics, a one-standard-deviation higher endurance predicts a 5.4% wage increase. This wage return to endurance is sizable, equivalent to a third of the wage return to ability. I also document positive associations between endurance and college attendance, college quality, college graduation, firm quality, and other outcomes. Finally, I show how systematic differences in endurance across students interact with the exam design to determine the sorting of students to colleges. I discuss the implications of these findings for the use of cognitive assessments for talent selection and investments in interventions that build cognitive endurance.

==> 7-exam-design-new.tex <==
\section{Endurance and the Sorting of Students to Colleges} \label{sec:equity-efficiency}

The sorting of students to colleges has important implications for the education and labor-market outcomes of these students \citep{macleod2017big}. In Brazil, as in many other countries, this sorting is largely mediated by admission exam scores. My results indicate that test scores reflect two valuable but distinct skills: ability and endurance. An important question is how these two skills contribute to the sorting of students to colleges. 

In this section, I estimate the effects of an exam reform that reduces the exam length by half. Such a reform would decrease the relative weight of endurance for determining test scores and increase the relative weight of ability. I focus on two channels through which the reform could affect the sorting of students to colleges. First, I study the \textit{distributional} effects of the reform, that is, how the reform would affect test-score gaps due to systematic differences in average endurance across types of students. Second, I study the \textit{informational} effects of the reform, that is, how the reform would affect the information on the quality of each applicant contained in test scores due to a change in the skills being measured by the exam. 


\subsection{Cognitive Endurance and Test-Score Gaps} \label{sub:correlates}

Standardized tests often exhibit large racial and income {test-score gaps} \citep[e.g.,][]{fryer2006black, card2007racial, riehl2022}. In the context of college admission exams, these gaps lead to inequitable college access and amplify earnings disparities \citep{chetty2020income}. An important question is what explains those test-score gaps. Next, I examine the contribution of differences in cognitive endurance to these gaps. 

\subsubsection{Decomposing Test-Score Gaps.}

To begin with, notice that the linear decomposition \eqref{reg:lpm-ind} can be used to parsimoniously summarize an individual's test score, $\text{TestScore}_i \equiv \E[C_{ij}]$, as a linear combination of her academic ability and endurance:

%
\begin{align} \label{eq:test-score}
	\text{TestScore}_i  = \hat{\alpha}_i + \hat{\beta}_i \overline{\text{Position}}.
\end{align}


Let $X \in \{0, 1\}$ be a student observable characteristic. For example, $X = 1$ may denote high-income students and $X = 0$ low-income students. The average test score of students with characteristic $x$ can be written as
%
\begin{align} \label{eq:test-score-grp}
	\E[\text{TestScore}_i | X_i = x]  = \E[\hat{\alpha}_i | X_i = x]  +  \E[\hat{\beta}_i | X_i = x] \overline{\text{Position}}.
\end{align}

Using this expression, the test-score gap, $\text{ScoreGap}$, can be decomposed into differences in average academic ability and differences in average cognitive endurance as follows:			
%
\begin{align} \label{eq:oaxaca}
	\text{ScoreGap} =  
	\underbrace{{\alpha}_{1} - {\alpha}_{0}}_{\substack{\text{Difference in average} \\ \text{academic ability} \\ \text{between groups}}} + 
	\underbrace{({\beta}_{1} - {\beta}_{0}) \overline{\text{Position}}}_{\substack{\text{Difference in average} \\ \text{cognitive endurance} \\ \text{between groups}}},
\end{align}
%
where $\alpha_x \equiv \E[\hat{\alpha}_i | X_i = x]$ and $\beta_x \equiv \E[\hat{\beta}_i | X_i = x]$. Equation \eqref{eq:oaxaca} shows that, in the absence of systematic differences in limited endurance ($\beta_1 = \beta_0$), test scores gaps would be purely a reflection of gaps in academic ability. Thus, exam design features that put a higher or lower weight on endurance, such as the length of the exam or the number of breaks, should not affect test-score gaps. This is no longer true in the presence of systematic differences in endurance. If student-level characteristics are associated with endurance, then an exam design that puts more weight on endurance will affect test-score gaps.  % In this case, the exam design impacts test scores by influencing $\hat{\beta}_i \overline{\text{Position}}$. 

I focus on estimating the impact of an exam reform that decreases the length of the test by half on test-score gaps.\footnote{Such a reform would be equivalent to changing the ENEM from its current length to roughly the length of the ACT exam.} This reform would decrease the average question position (from $\overline{\text{Position}}$ to $\overline{\text{Position}}/2$), thereby decreasing the influence of endurance gaps on test-score gaps.\footnote{An important concern is that, by reducing the number of questions, the exam would determine the place in the score distribution of any one student with less precision. However, the reform could be achieved without sacrificing much precision by using an adaptive exam that selects questions based on the student's ability level.} While I focus on test length, other exam features can also affect the influence of endurance for test-score gaps. For example, Figures \ref{fig:mean-corr}--\ref{fig:mean-corr-res} show that student performance starkly increases between the end of the first day and the beginning of the second day, suggesting that giving students more breaks would decrease the importance of endurance for test-scores gaps. Similarly, in Appendix \ref{app:het-question}, I show that the \textit{type} of exam questions impacts cognitive fatigue, thereby influencing the importance of endurance for test-score gaps. Thus, the reform can also be interpreted as, for example, introducing a long break in the middle of each testing day. %or as reducing by how mentally taxing each question is, for instance, by simplifying the wording of the prompt without changing the material tested.

% Identification assumption of the reform 

Using equation \eqref{eq:test-score}, I estimate the effects of the reform on test-score gaps between:

\begin{enumerate}
	\item Male and female students,
	\item White and non-white (Black, Brown, and Indigenous) students,
	\item Students in households in the top 30\% and bottom 30\% of the income distribution,
	\item Students with a college-educated mother and non-college-educated mother,
	\item Students enrolled in a private high school and public high school.
\end{enumerate}

\subsubsection{The Impact of an Exam Reform on Test-Score Gaps.}

Table \ref{tab:corr-endurance} shows estimates of the contribution of gaps in ability and endurance to test-score gaps. Column 1 shows the difference in average test scores between the groups of students listed in the row header, column 2 shows the difference in average academic ability (in a regression that controls for endurance), and column 3 shows the difference in average cognitive endurance (controlling for ability).

By reducing the contribution of endurance gaps to test-score gaps by half, the reform would: (i) Reduce the gender test-score gap by 0.85 percentage points (a 32\% decrease from the pre-reform gap of 2.6 percentage points); (ii) Reduce the racial test-score gap by 0.08 percentage points (a 14\% decrease from the pre-reform gap of 5.7 percentage points); and (iii) Reduce the SES test-score gap by 1.3--3.1 percentage points (a 13\%--16\% decrease from pre-reform gaps), depending on the SES measure.

The predicted impact of the exam reform is robust to (i) measuring the gaps in percentiles (Appendix Table \ref{tab:corr-rob-pctil}); (ii) Estimating ability and endurance with alternative specifications (Appendix Table \ref{tab:corr-rob-meas}); (iii) Using alternative measures of question difficulty when estimating ability and endurance (Appendix Table \ref{tab:corr-rob-diff}); (iv) Excluding individuals in the tails of the ability or endurance distributions (Appendix Table \ref{tab:corr-rob-samp}); and (v) Using precision-weighted estimates (Appendix Table \ref{tab:corr-rob-prec}).

\subsection{Cognitive Endurance and the Predictive Validity of Test Scores} \label{sub:fatigue-informational}

Admission officers use test scores to screen applicants because they are {informative} about which applicants will succeed in college. The standard approach to assess the informative content of an exam test is to calculate the cross-individual correlation between test scores and a long-run outcome that colleges want to screen their applicants based on (such as first-year college GPA or on-time graduation). This correlation is known as the \textit{predictive validity} of an exam \citep{rothstein2004college}. Next, I study how an exam's predictive validity depends on cognitive endurance.

\subsubsection{Decomposing Predictive Validity.} 

In the presence of limited endurance, features of the exam that affect the weight of endurance will affect the exam's predictive validity. To see this, notice that the predictive validity of test scores for outcome $Y$, $\rho^Y$, can be written as:
%
\begin{align} \label{eq:pred-val}
	\rho^Y  &\equiv \text{Corr}(Y_i, \text{TestScore}_i)   \notag \\
	        &= \text{Corr}(Y_i,  \alpha_i + \beta_i \overline{\text{Position}}) \notag \\
	        &= \frac{\sigma_{\alpha}}{\sigma_T} \text{Corr}(Y_i,\alpha_i) +  \frac{\sigma_{\beta}}{\sigma_T}\text{Corr}(Y_i,\beta_i)\overline{\text{Position}},
\end{align}
%
where $\sigma_{\alpha}, \sigma_{\beta}, \sigma_T$ are the standard deviations of ability, endurance, and test scores. Equation \eqref{eq:pred-val} shows that the predictive validity of an exam can be expressed as a linear combination of the correlation between the outcome and the skills measured by the exam. The weight of each skill depends on its dispersion and the exam's length. Unfortunately, equation \eqref{eq:pred-val} cannot be directly used to predict how an exam reform that changes the test length would affect its predictive validity, i.e.,  $\partial \rho^Y/\partial\overline{\text{Position}}$. This is because, as shown in Section \ref{sub:correlates}, such a reform would change the ranking of students, thereby affecting $\text{Corr}(Y_i,\alpha_i)$ and $\text{Corr}(Y_i,\beta_i)$.

I sidetrack this problem by studying how predictive validity varies throughout the exam. In particular, I ask how a given question's predictive validity $\rho^Y_j \equiv \text{Corr}(Y_i, C_{ij})$, changes when its position changes. Notice that the predictive validity of the overall exam can be written as a weighted average of the predictive validity of each exam question $j \in \{1, ..., J\}$:
%
\begin{align} \label{eq:pred-val-decomp}
	\rho^Y = \frac{1}{J} \sum_{j=1}^J  \frac{\sigma_{C_{ij}}}{\sigma_T} \rho^Y_j.
\end{align}
%
Equation \eqref{eq:pred-val-decomp} is helpful because it allows me to exploit the random variation in whether a given question is presented when students are relatively fresh or cognitively fatigued. To build intuition on the mechanics of this analysis, notice that $\rho^Y_j$ is given by the difference in average outcomes between students who correctly and incorrectly responded to question $j$, multiplied by the ratio of standard deviations:
%
\begin{align} \label{eq:pred-val-exp}
	\rho^Y_j = \Big(\E[Y_i | C_{ij} = 1] - \E[Y_i | C_{ij} = 0] \Big) \frac{\sigma_{C_{ij}}}{\sigma_{Y_{i}}}.
\end{align}


Equation \eqref{eq:pred-val-exp} indicates that limited endurance affects the predictive validity of a question by changing the composition of students who correctly answer the question. Loosely speaking, correct responses at the beginning of the exam are driven by high-ability students (regardless of their endurance level since all students are ``fresh'') and low-ability students who guessed the answer. Toward the end of the exam, correct responses are driven by students with high ability \textit{and} high cognitive endurance and students with either low ability \textit{or} low endurance who guessed the answer. 

How this compositional change affects a question's predictive power for an outcome is theoretically ambiguous. It depends on how the outcome correlates to academic ability relative to cognitive endurance, the distribution of ability and endurance in the population, and how difficult the question is. Thus, I empirically assess this by estimating regressions of the form:
%
\begin{align} \label{reg:validity-pos}
	\rho^Y_{jb} &= \alpha_j + \gamma^Y \text{Position}_{jb} + \eta_{jb}.
\end{align}
%
where $\rho^Y_{jb}$ is the predictive validity of question $j$ in booklet $b$, $\alpha_j$ are question fixed effects, and $\text{Position}_{jb}$ is the position of question $j$ in booklet $b$. The coefficient of interest is $\gamma^Y$, which measures the impact of a one-position increase in the order of a given question on the question's predictive validity for outcome $Y$. I scale $\gamma^Y$ so that it represents the change in predictive validity due to a reform that decreases the average question position by half.

I estimate the effect of the reform for eight main outcomes: test score (calculated without the contribution of question $j$ to avoid mechanical effects), college enrollment, college quality, degree progress, six-year graduation rate, hourly wage, monthly earnings, and firm leave-individual-out mean earnings. Since the dependent variable is an estimate, I weight each observation using the inverse square of its standard error. I cluster standard errors at the question position level.

%In the baseline regressions, I estimate the $\rho^Y_{jb}$'s without controls. To assess the robustness of the results, I also estimate $\rho^Y_{jb}$'s after controlling for student-level characteristics (age, gender, race, household income, high-school type, and municipality of residence).


\subsubsection{The Impact of an Exam Reform on the Test's Predictive Validity.} 

Table \ref{tab:val-pos} presents the results. Panel A shows the average predictive validity across all test questions. I find that individual questions are predictive of student long-run outcomes, although the size of the correlations tends to be small. For example, on average across all questions, correctly responding to a question has a 0.05 positive correlation with enrolling in college (column 2, $p < 0.01$), 0.10 correlation with college quality (column 3, $p < 0.01$), and 0.10 correlation with wages and earnings (columns 6--7, $p < 0.01$).

Panel B reports the estimates of equation \eqref{reg:validity-pos}. The exam reform would generate a sizable increase in the predictive validity of the exam for the majority of outcomes. For example, the exam reform would increase the average predictive validity of test responses for college enrollment by 0.05 points (a 95.2\% increase relative to the pre-reform mean, $p < 0.01$), for college quality by 0.09 points (a 91.1\% increase relative to the pre-reform mean), and for earnings by 0.07--0.08 points (a 75.7\%--79.6\% increase relative to the pre-reform mean, $p < 0.01$). The predicted effect for the six-year graduation rate is also positive but not statistically different from zero. The reform would decrease the predictive validity for degree progress.

These estimated effects of the reform are driven by the fact that a given question tends to be less predictive of long-run outcomes if it appears later in the exam. This can be seen visually in Appendix Figure \ref{fig:pred-val-chg-pos}, which shows binned scatterplots plotting the change in the predictive ability of a question ($y$-axis) against the change in the question position ($x$-axis) for selected outcomes. In all cases, the average predictive validity of test questions tends to decrease if the question appears later in the test.\footnote{The negative association can also be seen in Appendix Figure \ref{fig:pred-val-pos}, which plots the predictive validity of a question ($y$-axis) against its position on the exam ($x$-axis). There is an evident decline in predictive validity between the exam's beginning and end.}


%The results are qualitatively similar, although quantitatively smaller, when predictive validity is estimated including controls for student observable characteristics (Appendix Table \ref{tab:val-pos-rob-ctrl}).

% The new SAT was almost an hour longer
These results can help explain puzzling empirical findings in the literature. \cite{kobrin2008validity} study how the predictive validity of the SAT changed after the exam increased the number of questions in 2005. Intuitively, more test questions should lead to more precise student ability estimates and thus to more predictive test scores. Yet, the predictive validity of the exam did not change. This finding can be explained by cognitive fatigue eroding the predictive power of test responses at the end of the exam. \cite{bettinger2013improving} show that performance on the English and Math sections of the ACT predict college outcomes, but not performance on the Science and Reading sections. Based on this finding, the authors propose eliminating the Science and Reading sections. Notably, the Science and Reading questions are the last to appear in the ACT. Hence, the null predictive power of these two subjects may be driven by students being cognitively fatigued by the time they reach those sections---and not by the skills assessed by Science and Reading questions being irrelevant for long-run outcomes.\footnote{If the goal is to maximize the exam's predictive power, an alternative reform that might be more desirable is to reduce the number of questions in all sections (instead of eliminating some sections). Cognitive fatigue plays a smaller role in shorter tests, allowing students to reveal their academic preparedness across all questions. By not removing any subjects, colleges would have a measure of academic preparedness for all topics. I discuss the implications of my findings for exam design in Section \ref{sec:conclusions}.} 

\subsection{Discussion} 

In summary, this section shows that, due to heterogeneity in cognitive endurance, the design of college admission exams can have equity and efficiency consequences. I estimate that a reform that halves the exam length would reduce SES gaps by 26\%--29\%, possibly leading to a more diverse college student body. In addition, the shorter exam would be more informative about the quality of each applicant (as measured by its predictive validity), possibly leading to a better allocation of students to colleges. The first result is driven by the fact that, conditional on academic ability, low-SES students have lower endurance than high-SES students; thus, their performance declines at a steeper rate throughout the exam. The second result is driven by the fact that differences in student performance at the beginning of the exam mainly reflect differences in ability (roughly, because most students are ``fresh''), whereas performance differences towards the end of the exam increasingly reflect differences in endurance. Since ability is a stronger predictor of long-run outcomes than endurance, the predictive validity of a given question decreases if it appears later on the exam.
 

==> results/allq-pred-ctrl.tex <==
Constant&&0.002&\sym{***}&0.001&\sym{***}&0.002&\sym{***}&0.001&\sym{***}&0.001&\sym{***}&0.003&\sym{***}&0.003&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/allq-pred-item-N.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&\\


==> results/allq-pred-item-chg.tex <==
Slope/Mean&&$-$2.470&\sym{**}&$-$1.750&&$-$0.226&&2.756&\sym{***}&$-$3.250&&0.067&&$-$0.299&\\
&&(1.058&)&(1.131&)&(1.299&)&(1.017&)&(8.836&)&(1.048&)&(1.004&)\\


==> results/allq-pred-item.tex <==
Position (norm.)&&$-$0.006&\sym{**}&$-$0.003&&$-$0.001&&0.001&\sym{***}&$-$0.001&&0.000&&$-$0.001&\\
&&(0.003&)&(0.002&)&(0.004&)&(0.000&)&(0.004&)&(0.004&)&(0.004&)\\


==> results/allq-pred-pos-N.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&\\


==> results/allq-pred-pos-chg.tex <==
Slope/Constant&&$-$1.058&\sym{***}&$-$0.116&&1.627&\sym{*}&$-$1.267&\sym{***}&$-$1.431&\sym{***}&0.232&&0.699&\\
&&(0.101&)&(0.247&)&(0.858&)&(0.238&)&(0.181&)&(0.287&)&(0.482&)\\


==> results/allq-pred-pos-ctrl-N.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&\\


==> results/allq-pred-pos-ctrl-chg.tex <==
Slope/Constant&&$-$1.205&\sym{***}&$-$0.078&&1.780&\sym{**}&0.046&&$-$0.231&&0.186&&0.696&\sym{*}\\
&&(0.078&)&(0.181&)&(0.770&)&(0.397&)&(0.311&)&(0.248&)&(0.418&)\\


==> results/allq-pred-pos-ctrl.tex <==
Position (norm.)&&$-$0.005&\sym{***}&$-$0.000&&0.002&\sym{***}&0.000&&$-$0.000&&0.001&&0.001&\sym{**}\\
&&(0.001&)&(0.000&)&(0.001&)&(0.000&)&(0.000&)&(0.001&)&(0.001&)\\
Constant&&0.004&\sym{***}&0.002&\sym{***}&0.001&\sym{***}&0.001&\sym{***}&0.001&\sym{***}&0.003&\sym{***}&0.002&\sym{***}\\
&&(0.001&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/allq-pred-pos.tex <==
Position (norm.)&&$-$0.006&\sym{***}&$-$0.000&&0.003&\sym{***}&$-$0.001&\sym{***}&$-$0.002&\sym{***}&0.001&&0.002&\sym{**}\\
&&(0.001&)&(0.000&)&(0.001&)&(0.000&)&(0.001&)&(0.001&)&(0.001&)\\
Constant&&0.005&\sym{***}&0.002&\sym{***}&0.002&\sym{***}&0.001&\sym{***}&0.001&\sym{***}&0.004&\sym{***}&0.003&\sym{***}\\
&&(0.001&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.001&)&(0.001&)\\


==> results/allq-pred-power-N-beamer.tex <==
\(N\)&&180&&180&&180&&180&&180&\\


==> results/allq-pred-power-beamer.tex <==
Item position&&$-$0.047&\sym{***}&$-$0.009&\sym{***}&$-$0.005&\sym{***}&$-$0.010&\sym{***}&$-$0.025&\sym{***}\\
&&(0.006&)&(0.002&)&(0.001&)&(0.002&)&(0.004&)\\
Constant&&0.066&\sym{***}&0.033&\sym{***}&0.012&\sym{***}&0.019&\sym{***}&0.054&\sym{***}\\
&&(0.003&)&(0.001&)&(0.000&)&(0.001&)&(0.002&)\\


==> results/allq-pred-power-chg-beamer.tex <==
Change (in \%)&&$-$0.715&\sym{***}&$-$0.265&\sym{***}&$-$0.409&\sym{***}&$-$0.505&\sym{***}&$-$0.471&\sym{***}\\
&&(0.059&)&(0.065&)&(0.045&)&(0.065&)&(0.065&)\\


==> results/allq-pred.tex <==
Constant&&0.002&\sym{***}&0.002&\sym{***}&0.003&\sym{***}&0.000&\sym{**}&0.000&\sym{**}&0.004&\sym{***}&0.004&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/beta-coll-cred.tex <==
Cognitive Endurance ($\beta$)&&0.029&\sym{***}&0.042&\sym{***}&0.055&\sym{***}&0.062&\sym{***}\\
&&(0.000&)&(0.000&)&(0.001&)&(0.001&)\\
Academic Ability ($\alpha$)&&0.054&\sym{***}&0.079&\sym{***}&0.104&\sym{***}&0.117&\sym{***}\\
&&(0.000&)&(0.001&)&(0.001&)&(0.001&)\\
Mean Dep. Var.&&0.280&&0.400&&0.512&&0.590&\\
N&&1,001,107&&1,010,192&&1,014,053&&1,016,543&\\


==> results/beta-coll-enrol.tex <==
Cognitive Endurance ($\beta$)&&0.018&\sym{***}&0.019&\sym{***}&0.037&\sym{***}&9.505&\sym{***}\\
&&(0.001&)&(0.001&)&(0.000&)&(0.069&)\\
Academic Ability ($\alpha$)&&0.117&\sym{***}&0.124&\sym{***}&0.080&\sym{***}&19.755&\sym{***}\\
&&(0.001&)&(0.001&)&(0.000&)&(0.075&)\\
Mean Dep. Var.&&0.459&&0.491&&3.349&&540.045&\\
N&&1,812,353&&1,812,353&&883,428&&901,124&\\


==> results/beta-coll-grad.tex <==
Cognitive Endurance ($\beta$)&&0.002&\sym{***}&$-$0.013&\sym{***}&0.019&\sym{***}&$-$0.065&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.002&)\\
Academic Ability ($\alpha$)&&0.003&\sym{***}&$-$0.032&\sym{***}&0.047&\sym{***}&$-$0.147&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.002&)\\
Mean Dep. Var.&&0.220&&0.463&&0.469&&4.194&\\
N&&904,971&&904,971&&904,971&&446,987&\\


==> results/beta-coll-score.tex <==
Cognitive Endurance ($\beta$)&&$-$0.013&\sym{***}&$-$0.004&\sym{***}&$-$0.003&\sym{***}&$-$0.003&\sym{***}&$-$0.005&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.001&)&(0.001&)\\
Mean Dep. Var.&&0.511&&3.360&&0.093&&0.384&&0.431&\\
N&&1,152,999&&634,730&&647,459&&647,459&&647,459&\\


==> results/beta-coll.tex <==
Cognitive Endurance ($\beta$)&&0.070&\sym{***}&0.054&\sym{***}&$-$0.003&\sym{***}&0.018&\sym{***}&0.013&\sym{***}\\
&&(0.001&)&(0.000&)&(0.000&)&(0.001&)&(0.001&)\\
Adjusted Ability ($\alpha$)&&0.200&\sym{***}&0.114&\sym{***}&$-$0.001&&0.049&\sym{***}&0.044&\sym{***}\\
&&(0.001&)&(0.000&)&(0.001&)&(0.001&)&(0.001&)\\
Mean Dep. Var.&&0.511&&3.360&&0.093&&0.384&&0.431&\\
N&&1,153,906&&635,822&&648,463&&648,463&&648,463&\\


==> results/beta-ctrl-wage-N.tex <==
\(N\)&&819,046&&818,590&&811,646&&479,399&&479,221&&474,932&&474,780&&474,780&&396,542&\\
R$-$squared&&0.14&&0.23&&0.24&&0.29&&0.30&&0.38&&0.45&&0.49&&0.75&\\


==> results/beta-ctrl-wage-fs-N.tex <==
\(N\)&&396,549&&396,549&&396,549&&396,545&&396,539&&396,545&&396,545&&396,545&&396,542&\\
R$-$squared&&0.13&&0.21&&0.21&&0.28&&0.30&&0.38&&0.45&&0.49&&0.75&\\


==> results/beta-ctrl-wage-fs-shr.tex <==
Ratio coef.&&0.337&\sym{***}&0.351&\sym{***}&0.352&\sym{***}&0.364&\sym{***}&0.364&\sym{***}&0.330&\sym{***}&0.327&\sym{***}&0.326&\sym{***}&0.346&\sym{***}\\
&&(0.003&)&(0.003&)&(0.004&)&(0.004&)&(0.005&)&(0.006&)&(0.007&)&(0.007&)&(0.009&)\\


==> results/beta-ctrl-wage-fs.tex <==
Endurance&&0.077&\sym{***}&0.074&\sym{***}&0.071&\sym{***}&0.061&\sym{***}&0.053&\sym{***}&0.037&\sym{***}&0.031&\sym{***}&0.028&\sym{***}&0.020&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
Ability&&0.229&\sym{***}&0.211&\sym{***}&0.202&\sym{***}&0.168&\sym{***}&0.145&\sym{***}&0.112&\sym{***}&0.094&\sym{***}&0.086&\sym{***}&0.059&\sym{***}\\
&&(0.001&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)\\


==> results/beta-ctrl-wage-shr.tex <==
Ratio coef.&&0.331&\sym{***}&0.335&\sym{***}&0.336&\sym{***}&0.358&\sym{***}&0.358&\sym{***}&0.324&\sym{***}&0.321&\sym{***}&0.322&\sym{***}&0.346&\sym{***}\\
&&(0.002&)&(0.003&)&(0.003&)&(0.004&)&(0.004&)&(0.005&)&(0.006&)&(0.006&)&(0.009&)\\


==> results/beta-ctrl-wage.tex <==
Endurance&&0.079&\sym{***}&0.068&\sym{***}&0.064&\sym{***}&0.059&\sym{***}&0.051&\sym{***}&0.036&\sym{***}&0.030&\sym{***}&0.027&\sym{***}&0.020&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
Ability&&0.239&\sym{***}&0.202&\sym{***}&0.189&\sym{***}&0.166&\sym{***}&0.142&\sym{***}&0.112&\sym{***}&0.094&\sym{***}&0.084&\sym{***}&0.059&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.002&)&(0.002&)&(0.001&)&(0.001&)&(0.002&)\\


==> results/beta-labor.tex <==
Cognitive Endurance ($\beta$)&&$-$0.014&\sym{***}&0.052&\sym{***}&0.047&\sym{***}&$-$0.130&\sym{***}&0.000&\\
&&(0.001&)&(0.001&)&(0.001&)&(0.010&)&(0.001&)\\
Academic Ability ($\alpha$)&&$-$0.018&\sym{***}&0.138&\sym{***}&0.118&\sym{***}&$-$0.574&\sym{***}&0.016&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.011&)&(0.001&)\\
Mean Dep. Var.&&0.293&&3.825&&7.517&&41.034&&0.184&\\
N&&3,090,497&&902,798&&902,798&&906,815&&906,815&\\


==> results/ctrl-earn_mean-N.tex <==
\(N\)&&818,590&&811,646&&479,399&&479,221&&474,932&&474,780&&474,780&&396,542&\\
R$-$squared&&0.24&&0.24&&0.28&&0.30&&0.39&&0.47&&0.51&&0.76&\\


==> results/ctrl-earn_mean-fs-N.tex <==
\(N\)&&396,549&&396,549&&396,545&&396,539&&396,545&&396,545&&396,545&&396,542&\\
R$-$squared&&0.22&&0.22&&0.28&&0.30&&0.40&&0.48&&0.51&&0.76&\\


==> results/ctrl-earn_mean-fs-shr.tex <==
Ratio coef.&&0.353&\sym{***}&0.374&\sym{***}&0.385&\sym{***}&0.388&\sym{***}&0.406&\sym{***}&0.404&\sym{***}&0.350&\sym{***}&0.339&\sym{***}&0.337&\sym{***}&0.353&\sym{***}\\
&&(0.009&)&(0.003&)&(0.003&)&(0.004&)&(0.004&)&(0.004&)&(0.006&)&(0.007&)&(0.007&)&(0.009&)\\


==> results/ctrl-earn_mean-fs.tex <==
Endurance&&0.073&\sym{***}&0.070&\sym{***}&0.062&\sym{***}&0.058&\sym{***}&0.036&\sym{***}&0.029&\sym{***}&0.027&\sym{***}&0.019&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
Ability&&0.188&\sym{***}&0.181&\sym{***}&0.153&\sym{***}&0.143&\sym{***}&0.102&\sym{***}&0.086&\sym{***}&0.080&\sym{***}&0.055&\sym{***}\\
&&(0.001&)&(0.002&)&(0.001&)&(0.002&)&(0.002&)&(0.002&)&(0.001&)&(0.001&)\\


==> results/ctrl-earn_mean-shr.tex <==
Ratio coef.&&0.353&\sym{***}&0.360&\sym{***}&0.364&\sym{***}&0.367&\sym{***}&0.397&\sym{***}&0.395&\sym{***}&0.342&\sym{***}&0.332&\sym{***}&0.331&\sym{***}&0.353&\sym{***}\\
&&(0.009&)&(0.002&)&(0.003&)&(0.003&)&(0.004&)&(0.004&)&(0.005&)&(0.006&)&(0.006&)&(0.009&)\\


==> results/ctrl-earn_mean.tex <==
Endurance&&0.063&\sym{***}&0.060&\sym{***}&0.059&\sym{***}&0.055&\sym{***}&0.034&\sym{***}&0.028&\sym{***}&0.025&\sym{***}&0.019&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
Ability&&0.173&\sym{***}&0.162&\sym{***}&0.150&\sym{***}&0.139&\sym{***}&0.100&\sym{***}&0.084&\sym{***}&0.076&\sym{***}&0.055&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\


==> results/ctrl-wage-N.tex <==
\(N\)&&818,590&&811,646&&479,399&&479,221&&474,932&&474,780&&474,780&&396,542&\\
R$-$squared&&0.23&&0.24&&0.29&&0.30&&0.38&&0.45&&0.49&&0.75&\\


==> results/ctrl-wage-fs-N.tex <==
\(N\)&&396,549&&396,549&&396,545&&396,539&&396,545&&396,545&&396,545&&396,542&\\
R$-$squared&&0.21&&0.21&&0.28&&0.30&&0.38&&0.45&&0.49&&0.75&\\


==> results/ctrl-wage-fs-shr.tex <==
Ratio coef.&&0.346&\sym{***}&0.337&\sym{***}&0.351&\sym{***}&0.352&\sym{***}&0.364&\sym{***}&0.364&\sym{***}&0.330&\sym{***}&0.327&\sym{***}&0.326&\sym{***}&0.346&\sym{***}\\
&&(0.003&)&(0.003&)&(0.004&)&(0.004&)&(0.005&)&(0.006&)&(0.007&)&(0.007&)&(0.009&)\\


==> results/ctrl-wage-fs.tex <==
Endurance&&0.074&\sym{***}&0.071&\sym{***}&0.061&\sym{***}&0.053&\sym{***}&0.037&\sym{***}&0.031&\sym{***}&0.028&\sym{***}&0.020&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
Ability&&0.211&\sym{***}&0.202&\sym{***}&0.168&\sym{***}&0.145&\sym{***}&0.112&\sym{***}&0.094&\sym{***}&0.086&\sym{***}&0.059&\sym{***}\\
&&(0.002&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)&(0.002&)\\


==> results/ctrl-wage-shr.tex <==
Ratio coef.&&0.331&\sym{***}&0.335&\sym{***}&0.336&\sym{***}&0.358&\sym{***}&0.358&\sym{***}&0.324&\sym{***}&0.321&\sym{***}&0.322&\sym{***}&0.346&\sym{***}\\
&&(0.009&)&(0.002&)&(0.003&)&(0.003&)&(0.004&)&(0.004&)&(0.005&)&(0.006&)&(0.006&)&(0.009&)\\


==> results/ctrl-wage.tex <==
Endurance&&0.068&\sym{***}&0.064&\sym{***}&0.059&\sym{***}&0.051&\sym{***}&0.036&\sym{***}&0.030&\sym{***}&0.027&\sym{***}&0.020&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
Ability&&0.202&\sym{***}&0.189&\sym{***}&0.166&\sym{***}&0.142&\sym{***}&0.112&\sym{***}&0.094&\sym{***}&0.084&\sym{***}&0.059&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.002&)&(0.002&)&(0.001&)&(0.001&)&(0.002&)\\


==> results/endurance-N.tex <==
\(N\) (Students)&&14,941,097&&14,941,097&&14,941,097&\\


==> results/endurance-age.tex <==
age&&$-$0.004&\sym{***}&$-$0.004&\sym{***}&0.002&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-char.tex <==
Age&&$-$0.024&\sym{***}&$-$0.023&\sym{***}&0.005&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\
Male&&0.186&\sym{***}&0.062&\sym{***}&0.184&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)\\
White&&0.271&\sym{***}&0.206&\sym{***}&$-$0.027&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)\\
Private HS&&0.832&\sym{***}&0.730&\sym{***}&$-$0.143&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)\\
High income&&0.848&\sym{***}&0.646&\sym{***}&$-$0.013&\sym{***}\\
&&(0.002&)&(0.002&)&(0.002&)\\
\(N\)&&9705995&&9705995&&9705995&\\


==> results/endurance-ctl-age.tex <==
age&&$-$0.004&\sym{***}&$-$0.004&\sym{***}&$-$0.003&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-ctl-high_inc_5mw.tex <==
High income--Low income&&0.166&\sym{***}&0.162&\sym{***}&0.097&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-ctl-high_income.tex <==
High incom--Low income&&0.192&\sym{***}&0.188&\sym{***}&0.063&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-ctl-hs_priv.tex <==
Private-Public high school&&0.130&\sym{***}&0.127&\sym{***}&0.038&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-ctl-male.tex <==
Male-Female&&0.026&\sym{***}&0.030&\sym{***}&0.017&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-ctl-mom_coll.tex <==
Mom college-No college&&0.098&\sym{***}&0.095&\sym{***}&0.026&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-ctl-rank-age.tex <==
age&&$-$0.987&\sym{***}&$-$0.711&\sym{***}&$-$0.340&\sym{***}\\
&&(0.002&)&(0.001&)&(0.001&)\\


==> results/endurance-ctl-rank-high_inc_5mw.tex <==
High income--Low income&&33.008&\sym{***}&26.771&\sym{***}&18.589&\sym{***}\\
&&(0.023&)&(0.025&)&(0.031&)\\


==> results/endurance-ctl-rank-high_income.tex <==
High incom--Low income&&39.839&\sym{***}&31.775&\sym{***}&20.762&\sym{***}\\
&&(0.023&)&(0.024&)&(0.031&)\\


==> results/endurance-ctl-rank-hs_priv.tex <==
Private-Public high school&&27.827&\sym{***}&21.952&\sym{***}&13.255&\sym{***}\\
&&(0.019&)&(0.017&)&(0.020&)\\


==> results/endurance-ctl-rank-male.tex <==
Male-Female&&5.871&\sym{***}&5.599&\sym{***}&6.410&\sym{***}\\
&&(0.015&)&(0.012&)&(0.012&)\\


==> results/endurance-ctl-rank-mom_coll.tex <==
Mom college-No college&&21.609&\sym{***}&16.728&\sym{***}&9.191&\sym{***}\\
&&(0.018&)&(0.015&)&(0.016&)\\


==> results/endurance-ctl-rank-white.tex <==
White-Non-white&&14.127&\sym{***}&10.618&\sym{***}&6.193&\sym{***}\\
&&(0.015&)&(0.011&)&(0.012&)\\


==> results/endurance-ctl-white.tex <==
White-Non-white&&0.057&\sym{***}&0.056&\sym{***}&0.016&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-high_inc_5mw.tex <==
High income&&0.166&\sym{***}&0.176&\sym{***}&$-$0.022&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-high_income.tex <==
High incom$-$$-$Low income&&0.192&\sym{***}&0.206&\sym{***}&$-$0.014&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-hs_priv.tex <==
Private$-$Public high school&&0.130&\sym{***}&0.141&\sym{***}&$-$0.011&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-male.tex <==
Male$-$Female&&0.026&\sym{***}&0.013&\sym{***}&0.013&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-mom_coll.tex <==
Mom college$-$No college&&0.098&\sym{***}&0.108&\sym{***}&$-$0.010&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/endurance-rank-age.tex <==
age&&$-$0.987&\sym{***}&$-$0.853&\sym{***}&0.219&\sym{***}\\
&&(0.002&)&(0.002&)&(0.002&)\\


==> results/endurance-rank-high_inc_5mw.tex <==
High income&&33.008&\sym{***}&29.520&\sym{***}&$-$4.119&\sym{***}\\
&&(0.023&)&(0.025&)&(0.034&)\\


==> results/endurance-rank-high_income.tex <==
High incom--Low income&&39.839&\sym{***}&35.318&\sym{***}&-5.477&\sym{***}\\
&&(0.023&)&(0.025&)&(0.034&)\\


==> results/endurance-rank-hs_priv.tex <==
Private-Public high school&&27.827&\sym{***}&24.636&\sym{***}&-4.300&\sym{***}\\
&&(0.019&)&(0.020&)&(0.023&)\\


==> results/endurance-rank-male.tex <==
Male-Female&&5.871&\sym{***}&2.427&\sym{***}&4.822&\sym{***}\\
&&(0.015&)&(0.015&)&(0.015&)\\


==> results/endurance-rank-mom_coll.tex <==
Mom college-No college&&21.609&\sym{***}&19.220&\sym{***}&-3.935&\sym{***}\\
&&(0.018&)&(0.018&)&(0.020&)\\


==> results/endurance-rank-white.tex <==
White-Non-white&&14.127&\sym{***}&11.679&\sym{***}&-1.649&\sym{***}\\
&&(0.015&)&(0.015&)&(0.015&)\\


==> results/endurance-white.tex <==
White$-$Non$-$white&&0.057&\sym{***}&0.061&\sym{***}&$-$0.004&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-diff-ctrl0-N.tex <==
\(N\)&&14,941,097&&14,565,550&&9,924,652&&14,290,759&&9,996,959&\\


==> results/gap-diff-ctrl1-N.tex <==
\(N\)&&14,941,097&&14,565,550&&9,924,652&&14,290,759&&9,996,959&\\


==> results/gap-diff-ctrl3-N.tex <==
\(N\)&&14,941,097&&14,565,550&&9,924,652&&14,290,759&&9,996,959&\\


==> results/gap-diff-ctrl4-N.tex <==
\(N\)&&14,941,097&&14,565,550&&9,924,652&&14,290,759&&9,996,959&\\


==> results/gap-diff-ctrl5-N.tex <==
\(N\)&&14,941,097&&14,565,550&&9,924,652&&14,290,759&&9,996,959&\\


==> results/gap-diff-noctl-N.tex <==
\(N\)&&14,941,097&&14,565,550&&9,924,652&&14,290,759&&9,996,959&\\


==> results/gap-meas-day_avg-N.tex <==
\(N\)&&14,940,619&&14,565,087&&9,924,291&&14,290,307&&9,996,557&\\


==> results/gap-meas-day_fe-N.tex <==
\(N\)&&14,940,619&&14,565,087&&9,924,291&&14,290,307&&9,996,557&\\


==> results/gap-meas-rho-N.tex <==
\(N\)&&14,941,097&&14,565,550&&9,924,652&&14,290,759&&9,996,959&\\


==> results/gap-meas-shrink-N.tex <==
\(N\)&&11,577,409&&11,273,866&&7,523,921&&11,031,888&&7,662,542&\\


==> results/gap-meas-subj_avg-N.tex <==
\(N\)&&14,939,785&&14,564,280&&9,923,669&&14,289,518&&9,995,909&\\


==> results/gap-meas-subj_fe-N.tex <==
\(N\)&&14,939,785&&14,564,280&&9,923,669&&14,289,518&&9,995,909&\\


==> results/gap-meas-wt-N.tex <==
\(N\)&&14,941,097&&14,565,550&&9,924,652&&14,290,759&&9,996,959&\\


==> results/gap-rest-N.tex <==
\(N\) (Students)&&2,418,766&&2,354,955&&1,661,467&&2,363,282&&1,245,415&\\


==> results/gap-rest-alpha.tex <==
Ability gap&&0.002&\sym{***}&0.008&\sym{***}&0.020&\sym{***}&0.015&\sym{***}&0.027&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-rest-beta.tex <==
Endurance gap&&0.027&\sym{***}&0.022&\sym{***}&0.039&\sym{***}&0.028&\sym{***}&0.053&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-rest-pct.tex <==
Pct. change gap&&-0.521&\sym{***}&-0.189&\sym{***}&-0.151&\sym{***}&-0.141&\sym{***}&-0.138&\sym{***}\\
&&(0.002&)&(0.001&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-rest-pct_corr.tex <==
Test-score gap&&0.030&\sym{***}&0.030&\sym{***}&0.059&\sym{***}&0.043&\sym{***}&0.081&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-rest-pp.tex <==
P.p. change gap&&-0.014&\sym{***}&-0.011&\sym{***}&-0.020&\sym{***}&-0.014&\sym{***}&-0.026&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-samp-alpha10-N.tex <==
\(N\)&&11,952,877&&11,663,864&&7,924,866&&11,431,969&&8,053,826&\\


==> results/gap-samp-alpha20-N.tex <==
\(N\)&&8,964,659&&8,751,160&&5,955,592&&8,572,079&&6,097,095&\\


==> results/gap-samp-alpha20-alpha.tex <==
Ability gap&&0.010&\sym{***}&0.023&\sym{***}&0.044&\sym{***}&0.031&\sym{***}&0.070&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-samp-alpha20-beta.tex <==
Endurance gap&&0.031&\sym{***}&0.030&\sym{***}&0.063&\sym{***}&0.043&\sym{***}&0.101&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-samp-beta10-N.tex <==
\(N\)&&11,952,877&&11,655,032&&7,923,646&&11,417,917&&8,131,223&\\


==> results/gap-samp-beta20-N.tex <==
\(N\)&&8,964,657&&8,741,118&&5,937,755&&8,557,424&&6,143,268&\\


==> results/gap-samp-beta20-alpha.tex <==
Ability gap&&0.026&\sym{***}&0.054&\sym{***}&0.125&\sym{***}&0.094&\sym{***}&0.191&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-samp-beta20-beta.tex <==
Endurance gap&&0.009&\sym{***}&0.010&\sym{***}&0.023&\sym{***}&0.016&\sym{***}&0.046&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)\\


==> results/gap-samp-betapos-N.tex <==
\(N\)&&9,693,476&&9,454,492&&6,415,899&&9,293,758&&6,384,954&\\


==> results/gap-samp-both10-N.tex <==
\(N\)&&10,386,454&&10,134,002&&6,871,467&&9,920,393&&7,081,924&\\


==> results/gap-samp-both20-N.tex <==
\(N\)&&6,534,980&&6,377,150&&4,331,259&&6,237,046&&4,506,484&\\


==> results/ind-pred-pos-beamer.tex <==
Item position&&$-$0.047&\sym{***}&$-$0.009&\sym{***}&$-$0.005&\sym{***}&$-$0.010&\sym{***}&$-$0.025&\sym{***}\\
&&(0.006&)&(0.002&)&(0.001&)&(0.002&)&(0.004&)\\
Constant&&0.066&\sym{***}&0.033&\sym{***}&0.012&\sym{***}&0.019&\sym{***}&0.054&\sym{***}\\
&&(0.003&)&(0.001&)&(0.000&)&(0.001&)&(0.002&)\\


==> results/indq-pred-ctrl.tex <==
Constant&&0.249&\sym{***}&0.039&\sym{***}&0.070&\sym{***}&0.058&\sym{***}&0.026&\sym{***}&0.020&\sym{***}&0.065&\sym{***}&0.061&\sym{***}\\
&&(0.006&)&(0.001&)&(0.002&)&(0.001&)&(0.001&)&(0.001&)&(0.002&)&(0.002&)\\


==> results/indq-pred-item-N-beamer.tex <==
\(N\) (Items)&&1,416&&1,416&&1,416&&1,416&&1,416&\\


==> results/indq-pred-item-N.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&\\


==> results/indq-pred-item-beamer.tex <==
Position (norm.)&&$-$0.080&\sym{**}&$-$0.070&\sym{***}&$-$0.052&\sym{***}&$-$0.038&\sym{**}&$-$0.037&\sym{**}\\
&&(0.033&)&(0.023&)&(0.017&)&(0.016&)&(0.017&)\\


==> results/indq-pred-item-chg-beamer.tex <==
Slope/Mean&&$-$0.276&\sym{**}&$-$0.484&\sym{***}&$-$0.427&\sym{***}&$-$0.359&\sym{**}&$-$0.355&\sym{**}\\
&&(0.115&)&(0.160&)&(0.142&)&(0.149&)&(0.163&)\\


==> results/indq-pred-item-chg.tex <==
Slope/Mean&&$-$0.517&\sym{***}&$-$0.566&\sym{***}&$-$0.471&\sym{***}&$-$0.314&\sym{***}&$-$3.663&\sym{***}&$-$1.373&\sym{***}&$-$0.535&\sym{***}&$-$0.485&\sym{***}\\
&&(0.091&)&(0.100&)&(0.101&)&(0.099&)&(0.742&)&(0.163&)&(0.104&)&(0.105&)\\


==> results/indq-pred-item-cons-beamer.tex <==
Constant&&0.268&\sym{***}&0.142&\sym{***}&0.121&\sym{***}&0.107&\sym{***}&0.103&\sym{***}\\
&&(0.008&)&(0.005&)&(0.003&)&(0.003&)&(0.003&)\\


==> results/indq-pred-item-ctrl-N.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&\\


==> results/indq-pred-item-ctrl-chg.tex <==
Slope/Constant&&$-$0.148&&$-$0.378&\sym{***}&$-$0.334&\sym{***}&$-$0.225&\sym{*}&$-$0.103&&$-$0.124&&$-$0.299&\sym{**}&$-$0.274&\sym{*}\\
&&(0.108&)&(0.113&)&(0.099&)&(0.134&)&(0.073&)&(0.296&)&(0.138&)&(0.140&)\\


==> results/indq-pred-item-ctrl.tex <==
Position (norm.)&&$-$0.040&&$-$0.018&\sym{***}&$-$0.028&\sym{***}&$-$0.015&&$-$0.003&&$-$0.003&&$-$0.023&\sym{*}&$-$0.019&\sym{*}\\
&&(0.031&)&(0.007&)&(0.010&)&(0.010&)&(0.002&)&(0.007&)&(0.012&)&(0.011&)\\


==> results/indq-pred-item-mean-beamer.tex <==
Mean Dep. Var.&&5.332&&3.434&&1.001&&1.666&&4.951&\\


==> results/indq-pred-item-mean.tex <==
Mean Dep. Var.&&0.268&&0.142&&0.121&&0.016&&0.103&&0.099&&0.083&&0.076&\\


==> results/indq-pred-item-tex.tex <==
Position (norm.)&&$-$0.000&&$-$0.019&\sym{***}&$-$0.001&&$-$0.002&&0.004&\sym{*}&$-$0.010&\sym{***}\\
&&(0.010&)&(0.005&)&(0.004&)&(0.002&)&(0.002&)&(0.003&)\\


==> results/indq-pred-item.tex <==
Position (norm.)&&$-$0.058&\sym{*}&$-$0.027&\sym{***}&$-$0.050&\sym{***}&$-$0.037&\sym{**}&0.003&\sym{**}&$-$0.002&&$-$0.042&\sym{**}&$-$0.038&\sym{**}\\
&&(0.035&)&(0.009&)&(0.016&)&(0.015&)&(0.001&)&(0.006&)&(0.017&)&(0.016&)\\


==> results/indq-pred-pos-N-beamer.tex <==
\(N\)&&180&&180&&180&&180&&180&\\


==> results/indq-pred-pos-N-stud.tex <==
\(N\) (Students)&&1,416&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&\\


==> results/indq-pred-pos-N.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&\\


==> results/indq-pred-pos-beamer.tex <==
Item position&&$-$0.047&\sym{***}&$-$0.009&\sym{***}&$-$0.005&\sym{***}&$-$0.010&\sym{***}&$-$0.025&\sym{***}\\
&&(0.006&)&(0.002&)&(0.001&)&(0.002&)&(0.004&)\\
Constant&&0.066&\sym{***}&0.033&\sym{***}&0.012&\sym{***}&0.019&\sym{***}&0.054&\sym{***}\\
&&(0.003&)&(0.001&)&(0.000&)&(0.001&)&(0.002&)\\


==> results/indq-pred-pos-chg-beamer.tex <==
Change (in \%)&&$-$0.715&\sym{***}&$-$0.265&\sym{***}&$-$0.409&\sym{***}&$-$0.505&\sym{***}&$-$0.471&\sym{***}\\
&&(0.059&)&(0.065&)&(0.045&)&(0.065&)&(0.065&)\\


==> results/indq-pred-pos-chg.tex <==
Slope/Constant&&$-$0.413&\sym{***}&$-$0.440&\sym{***}&$-$0.381&\sym{***}&$-$0.272&\sym{***}&$-$1.274&\sym{***}&$-$0.809&\sym{***}&$-$0.423&\sym{***}&$-$0.391&\sym{***}\\
&&(0.058&)&(0.060&)&(0.066&)&(0.074&)&(0.081&)&(0.055&)&(0.065&)&(0.068&)\\


==> results/indq-pred-pos-ctrl-N.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&\\


==> results/indq-pred-pos-ctrl-chg.tex <==
Slope/Constant&&$-$0.466&\sym{***}&$-$0.526&\sym{***}&$-$0.422&\sym{***}&$-$0.272&\sym{***}&$-$0.446&\sym{***}&$-$0.608&\sym{***}&$-$0.463&\sym{***}&$-$0.418&\sym{***}\\
&&(0.052&)&(0.052&)&(0.060&)&(0.070&)&(0.088&)&(0.065&)&(0.059&)&(0.063&)\\


==> results/indq-pred-pos-ctrl.tex <==
Position (norm.)&&$-$0.151&\sym{***}&$-$0.028&\sym{***}&$-$0.038&\sym{***}&$-$0.018&\sym{***}&$-$0.015&\sym{***}&$-$0.017&\sym{***}&$-$0.039&\sym{***}&$-$0.032&\sym{***}\\
&&(0.021&)&(0.004&)&(0.007&)&(0.005&)&(0.004&)&(0.003&)&(0.006&)&(0.006&)\\
Constant&&0.324&\sym{***}&0.053&\sym{***}&0.089&\sym{***}&0.067&\sym{***}&0.033&\sym{***}&0.028&\sym{***}&0.084&\sym{***}&0.077&\sym{***}\\
&&(0.011&)&(0.002&)&(0.004&)&(0.003&)&(0.002&)&(0.002&)&(0.004&)&(0.003&)\\


==> results/indq-pred-pos.tex <==
Position (norm.)&&$-$0.148&\sym{***}&$-$0.033&\sym{***}&$-$0.051&\sym{***}&$-$0.030&\sym{***}&$-$0.012&\sym{***}&$-$0.022&\sym{***}&$-$0.057&\sym{***}&$-$0.049&\sym{***}\\
&&(0.025&)&(0.006&)&(0.011&)&(0.009&)&(0.002&)&(0.003&)&(0.011&)&(0.010&)\\
Constant&&0.357&\sym{***}&0.074&\sym{***}&0.135&\sym{***}&0.112&\sym{***}&0.010&\sym{***}&0.027&\sym{***}&0.134&\sym{***}&0.126&\sym{***}\\
&&(0.013&)&(0.003&)&(0.006&)&(0.005&)&(0.001&)&(0.002&)&(0.006&)&(0.006&)\\


==> results/indq-pred.tex <==
Constant&&0.285&\sym{***}&0.057&\sym{***}&0.109&\sym{***}&0.097&\sym{***}&0.003&\sym{***}&0.016&\sym{***}&0.106&\sym{***}&0.101&\sym{***}\\
&&(0.007&)&(0.002&)&(0.003&)&(0.003&)&(0.001&)&(0.001&)&(0.003&)&(0.003&)\\


==> results/indq-reform-N-beamer.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&1,416&&1,416&\\


==> results/indq-reform-above-N.tex <==
\(N\) (Item$-$Booklets)&&468&&468&&468&&140&&468&&576&&576&&576&\\


==> results/indq-reform-above-chg.tex <==
Slope/Constant&&$-$0.414&\sym{***}&$-$0.534&\sym{***}&$-$0.385&\sym{***}&$-$1.908&\sym{***}&$-$1.869&\sym{***}&$-$0.052&&0.025&&$-$0.143&\sym{**}\\
&&(0.043&)&(0.068&)&(0.054&)&(0.514&)&(0.245&)&(0.048&)&(0.050&)&(0.059&)\\


==> results/indq-reform-above-cons.tex <==
Avg. Validity&&0.367&\sym{***}&0.067&\sym{***}&0.131&\sym{***}&0.013&\sym{***}&0.031&\sym{***}&0.108&\sym{***}&0.099&\sym{***}&0.091&\sym{***}\\
&&(0.008&)&(0.002&)&(0.003&)&(0.001&)&(0.001&)&(0.004&)&(0.004&)&(0.003&)\\


==> results/indq-reform-above.tex <==
Position (norm.)&&$-$0.142&\sym{***}&$-$0.033&\sym{***}&$-$0.047&\sym{***}&$-$0.019&\sym{***}&$-$0.045&\sym{***}&$-$0.006&&0.002&&$-$0.013&\\
&&(0.034&)&(0.006&)&(0.014&)&(0.006&)&(0.008&)&(0.009&)&(0.008&)&(0.009&)\\


==> results/indq-reform-beamer.tex <==
Chg. in Pred. Val.&&0.115&\sym{*}&0.055&\sym{***}&0.099&\sym{***}&0.084&\sym{**}&0.077&\sym{**}\\
&&(0.069&)&(0.018&)&(0.032&)&(0.034&)&(0.032&)\\


==> results/indq-reform-below-N.tex <==
\(N\) (Item$-$Booklets)&&1,648&&1,648&&1,648&&560&&1,648&&2,240&&2,240&&2,240&\\


==> results/indq-reform-below-chg.tex <==
Slope/Constant&&0.207&\sym{***}&0.156&\sym{***}&0.240&\sym{***}&$-$2.872&&0.261&&0.339&\sym{***}&0.352&\sym{***}&0.313&\sym{***}\\
&&(0.025&)&(0.046&)&(0.033&)&(6.182&)&(0.175&)&(0.032&)&(0.033&)&(0.038&)\\


==> results/indq-reform-below-cons.tex <==
Avg. Validity&&0.269&\sym{***}&0.047&\sym{***}&0.108&\sym{***}&0.001&&0.012&\sym{***}&0.069&\sym{***}&0.063&\sym{***}&0.060&\sym{***}\\
&&(0.007&)&(0.001&)&(0.003&)&(0.001&)&(0.001&)&(0.002&)&(0.002&)&(0.002&)\\


==> results/indq-reform-below.tex <==
Position (norm.)&&0.059&\sym{***}&0.008&\sym{**}&0.028&\sym{***}&$-$0.002&&0.003&&0.026&\sym{***}&0.025&\sym{***}&0.021&\sym{***}\\
&&(0.015&)&(0.003&)&(0.007&)&(0.002&)&(0.003&)&(0.004&)&(0.004&)&(0.004&)\\


==> results/indq-reform-chg-beamer.tex <==
Chg. Val./Mean&&0.404&\sym{***}&0.952&\sym{***}&0.911&\sym{***}&0.796&\sym{***}&0.757&\sym{***}\\
&&(0.110&)&(0.191&)&(0.144&)&(0.193&)&(0.194&)\\


==> results/indq-reform-cons-beamer.tex <==
Constant&&0.285&\sym{***}&0.057&\sym{***}&0.109&\sym{***}&0.106&\sym{***}&0.101&\sym{***}\\
&&(0.007&)&(0.002&)&(0.003&)&(0.003&)&(0.003&)\\


==> results/indq-reform-ctrl-N.tex <==
\(N\) (Item$-$Booklets)&&1,416&&1,416&&1,416&&700&&1,416&&1,416&&1,416&&1,416&\\


==> results/indq-reform-ctrl-chg.tex <==
Slope/Constant&&0.295&\sym{***}&0.756&\sym{***}&0.668&\sym{***}&0.207&\sym{**}&0.249&&0.598&\sym{***}&0.547&\sym{**}&0.648&\sym{**}\\
&&(0.102&)&(0.171&)&(0.120&)&(0.088&)&(0.491&)&(0.204&)&(0.213&)&(0.258&)\\


==> results/indq-reform-ctrl-cons.tex <==
Constant&&0.249&\sym{***}&0.039&\sym{***}&0.070&\sym{***}&0.026&\sym{***}&0.020&\sym{***}&0.065&\sym{***}&0.061&\sym{***}&0.052&\sym{***}\\
&&(0.006&)&(0.001&)&(0.002&)&(0.001&)&(0.001&)&(0.002&)&(0.002&)&(0.001&)\\


==> results/indq-reform-ctrl.tex <==
Position (norm.)&&0.079&&0.036&\sym{***}&0.057&\sym{***}&0.006&&0.005&&0.046&\sym{*}&0.039&\sym{*}&0.040&\sym{*}\\
&&(0.063&)&(0.013&)&(0.020&)&(0.004&)&(0.013&)&(0.025&)&(0.023&)&(0.023&)\\


==> results/oaxaca-N.tex <==
\(N\) (Students) &6,564,973 &9,633,475 &9,898,074 &9,451,905 \\


==> results/oaxaca-beamer.tex <==
Performance advantaged &0.523 &0.378 &0.450 &0.437 \\
Performance disadvantaged &0.312 &0.321 &0.320 &0.331 \\
Performance gap &0.211 &0.056 &0.130 &0.106 \\ \midrule
Contribution adjusted-ability  &0.230 &0.070 &0.151 &0.123 \\
 &(0.000) &(0.000) &(0.000) &(0.000) \\
Contribution fatigue &-0.026 &-0.013 &-0.023 &-0.018 \\
 &(0.000) &(0.000) &(0.000) &(0.000) \\
Change in gap due to fatigue &-0.125 &-0.238 &-0.180 &-0.173 \\ \midrule
N &6,564,973 &9,633,475 &9,898,074 &9,451,905 \\


==> results/oaxaca-decomp.tex <==
Fatigue-adjusted academic ability  &0.230 &0.070 &0.151 &0.123 \\
 &(0.000) &(0.000) &(0.000) &(0.000) \\
Cognitive endurance &-0.026 &-0.013 &-0.023 &-0.018 \\
 &(0.000) &(0.000) &(0.000) &(0.000) \\


==> results/oaxaca-mean.tex <==
Test score high-SES group &0.523 &0.378 &0.450 &0.437 \\
Test score low-SES group &0.312 &0.321 &0.320 &0.331 \\
Test score gap &0.211 &0.056 &0.130 &0.106 \\


==> results/oaxaca.tex <==
Performance advantaged group &0.523 &0.378 &0.450 &0.437 &0.365 \\
Performance Disadvantaged group &0.312 &0.321 &0.320 &0.331 &0.337 \\
Performance gap &0.211 &0.056 &0.130 &0.106 &0.028 \\ \midrule
contribution adjusted-ability  &0.230 &0.070 &0.151 &0.123 &0.018 \\
 &(0.000) &(0.000) &(0.000) &(0.000) &(0.000) \\
contribution cognitive fatigue  &-0.026 &-0.013 &-0.023 &-0.018 &0.011 \\
 &(0.000) &(0.000) &(0.000) &(0.000) &(0.000) \\
Change in gap due to fatigue &-0.125 &-0.238 &-0.180 &-0.173 &0.378 \\ \midrule
N &6,564,973 &9,633,475 &9,898,074 &9,451,905 &9,899,720 \\
 &. &. &. &. &. \\


==> results/pct-coll.tex <==
Test score&&0.174&\sym{***}&0.091&\sym{***}&$-$0.000&&0.043&\sym{***}&0.040&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.001&)&(0.001&)\\
Mean Dep. Var.&&0.511&&3.360&&0.093&&0.384&&0.431&\\
N&&1,153,909&&635,822&&648,463&&648,463&&648,463&\\


==> results/reg-N-beamer.tex <==
Mean DV&&0.244&&3.326&&0.158&&0.418&&3.865&\\
\(N\)&&2,501,522&&1,800,546&&1,124,972&&1,472,916&&818,590&\\


==> results/reg-beta-beamer.tex <==
Ability&&0.102&\sym{***}&0.095&\sym{***}&0.016&\sym{***}&0.072&\sym{***}&0.154&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.001&)&(0.001&)\\
Endurance&&0.032&\sym{***}&0.030&\sym{***}&0.006&\sym{***}&0.026&\sym{***}&0.054&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.001&)\\


==> results/reg-coll-beta-fe.tex <==
Cognitive Endurance ($\beta$)&&$-$0.014&\sym{***}&$-$0.005&\sym{***}&0.002&&$-$0.001&&0.026&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.002&)&(0.010&)\\
Mean Dep. Var.&&0.507&&3.357&&0.908&&0.384&&4.225&\\
N&&112,768&&59,596&&60,885&&60,885&&27,492&\\


==> results/reg-coll-rob-fe.tex <==
Cognitive Endurance&&$-$0.139&\sym{***}&0.055&\sym{***}&$-$0.025&\sym{**}&$-$0.121&\sym{***}&0.428&\sym{***}\\
&&(0.012&)&(0.010&)&(0.011&)&(0.018&)&(0.094&)\\


==> results/reg-earn_mean-ctrl-fs.tex <==
Endurance&&0.073&\sym{***}&0.070&\sym{***}&0.062&\sym{***}&0.058&\sym{***}&0.036&\sym{***}&0.029&\sym{***}&0.027&\sym{***}&0.019&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
Ability&&0.188&\sym{***}&0.181&\sym{***}&0.153&\sym{***}&0.143&\sym{***}&0.102&\sym{***}&0.086&\sym{***}&0.080&\sym{***}&0.055&\sym{***}\\
&&(0.001&)&(0.002&)&(0.001&)&(0.002&)&(0.002&)&(0.002&)&(0.001&)&(0.001&)\\
\(N\)&&396,549&&396,549&&396,545&&396,539&&396,545&&396,545&&396,545&&396,542&\\
R$-$squared&&0.22&&0.22&&0.28&&0.30&&0.40&&0.48&&0.51&&0.76&\\


==> results/reg-earn_mean-ctrl.tex <==
Endurance&&0.063&\sym{***}&0.060&\sym{***}&0.059&\sym{***}&0.055&\sym{***}&0.034&\sym{***}&0.028&\sym{***}&0.025&\sym{***}&0.019&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
Ability&&0.173&\sym{***}&0.162&\sym{***}&0.150&\sym{***}&0.139&\sym{***}&0.100&\sym{***}&0.084&\sym{***}&0.076&\sym{***}&0.055&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\
\(N\)&&818,590&&811,646&&479,399&&479,221&&474,932&&474,780&&474,780&&396,542&\\
R$-$squared&&0.24&&0.24&&0.28&&0.30&&0.39&&0.47&&0.51&&0.76&\\


==> results/reg-pct_corr-beamer.tex <==
Test score&&0.088&\sym{***}&0.082&\sym{***}&0.014&\sym{***}&0.060&\sym{***}&0.129&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.001&)&(0.001&)\\


==> results/reg-pos-corr-N.tex <==
\(N\) (Item$-$Booklets)&&5,896&&5,896&&5,896&\\


==> results/reg-pos-corr-N_r-beamer.tex <==
\(N\) (Responses)&&2,689,345,707&&2,689,345,707&&2,689,345,707&\\
R$-$squared&&0.85&&0.99&&0.97&\\


==> results/reg-pos-corr-beamer.tex <==
Position (norm.)&&$-$0.214&\sym{***}&$-$0.071&\sym{***}&$-$0.058&\sym{***}\\
&&(0.013&)&(0.004&)&(0.002&)\\
Constant&&0.450&\sym{***}&&&&\\
&&(0.008&)&&&&\\


==> results/reg-pos-stud-N.tex <==
\(N\) (Item$-$Booklets)&&5,896&&5,896&&5,896&&5,896&&5,896&&5,896&&5,896&&5,896&\\


==> results/reg-pos-stud.tex <==
Position (normalized)&&$-$0.061&\sym{***}&$-$0.104&\sym{***}&$-$0.067&\sym{***}&$-$0.092&\sym{***}&$-$0.064&\sym{***}&$-$0.088&\sym{***}&$-$0.066&\sym{***}&$-$0.078&\sym{***}\\
&&(0.004&)&(0.005&)&(0.004&)&(0.005&)&(0.004&)&(0.004&)&(0.004&)&(0.004&)\\


==> results/reg-que-pos.tex <==
Question position (normalized)&&$-$0.214&\sym{***}\\
&&(0.012&)\\
Constant&&0.453&\sym{***}\\
&&(0.006&)\\
\(N\)&&5896&\\


==> results/rob-samp-coll-alpha20.tex <==
Endurance&&0.031&\sym{***}&0.025&\sym{***}&0.034&\sym{***}&0.007&\sym{***}&0.033&\sym{***}&$-$0.049&\sym{***}\\
&&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.000&)&(0.002&)\\
Ability&&0.099&\sym{***}&0.078&\sym{***}&0.093&\sym{***}&0.021&\sym{***}&0.096&\sym{***}&$-$0.150&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.000&)&(0.001&)&(0.004&)\\


==> results/rob-samp-coll-beta20.tex <==
Endurance&&0.030&\sym{***}&0.031&\sym{***}&0.050&\sym{***}&0.006&\sym{***}&0.025&\sym{***}&$-$0.042&\sym{***}\\
&&(0.000&)&(0.000&)&(0.001&)&(0.000&)&(0.001&)&(0.002&)\\
Ability&&0.099&\sym{***}&0.092&\sym{***}&0.133&\sym{***}&0.016&\sym{***}&0.077&\sym{***}&$-$0.137&\sym{***}\\
&&(0.000&)&(0.000&)&(0.001&)&(0.000&)&(0.001&)&(0.003&)\\


==> results/rob-samp-lmkt-alpha20.tex <==
Endurance&&0.000&\sym{***}&0.043&\sym{***}&0.041&\sym{***}&0.029&\sym{***}&0.017&\sym{***}&0.004&\sym{***}\\
&&(0.000&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.000&)\\
Ability&&0.001&\sym{***}&0.120&\sym{***}&0.106&\sym{***}&0.086&\sym{***}&0.052&\sym{***}&0.016&\sym{***}\\
&&(0.000&)&(0.002&)&(0.002&)&(0.002&)&(0.001&)&(0.001&)\\


==> results/rob-samp-lmkt-beta20.tex <==
Endurance&&0.000&\sym{***}&0.050&\sym{***}&0.048&\sym{***}&0.033&\sym{***}&0.015&\sym{***}&0.003&\sym{***}\\
&&(0.000&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.000&)\\
Ability&&0.001&\sym{***}&0.146&\sym{***}&0.129&\sym{***}&0.102&\sym{***}&0.048&\sym{***}&0.014&\sym{***}\\
&&(0.000&)&(0.002&)&(0.001&)&(0.001&)&(0.001&)&(0.000&)\\


==> results/score-ctrl-wage-fs.tex <==
Test score&&0.193&\sym{***}&0.177&\sym{***}&0.169&\sym{***}&0.140&\sym{***}&0.120&\sym{***}&0.095&\sym{***}&0.080&\sym{***}&0.073&\sym{***}&0.050&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\


==> results/score-ctrl-wage.tex <==
Test score&&0.202&\sym{***}&0.171&\sym{***}&0.160&\sym{***}&0.139&\sym{***}&0.119&\sym{***}&0.095&\sym{***}&0.080&\sym{***}&0.071&\sym{***}&0.050&\sym{***}\\
&&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)&(0.001&)\\

